Unimodality for Radon partitions of random vectors

Consider the (almost surely) unique Radon partition of a set of $n$ random Gaussian vectors in $\mathbb R^{n-2}$; choose one of the two parts of this partition uniformly at random, and for $0 \le k \le n$, let $p_k$ denote the probability that it has size $k$. In this paper, we prove strong unimodality results for the distribution $(p_0,\dots,p_n)$.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Macros by Swee Hong

%%%%%%%%%% Standard macros
\DeclareMathOperator{\bX}{\bar{X}} % Sample mean
\DeclareMathOperator{\bY}{\bar{Y}} % Sample mean
\DeclareMathOperator{\bZ}{\bar{Z}} % Sample mean
\DeclareMathOperator{\Cov}{\textnormal{Cov}} % Covariance
\DeclareMathOperator{\Eb}{\mathbb{E}} % Expectation
\DeclareMathOperator{\Pb}{\mathbb{P}} % Probability measure
\DeclareMathOperator{\rr}{\mathbb{R}} % Real numbers
\DeclareMathOperator{\cC}{\mathcal{C}} % Real numbers

%%%%%%%%%% Local macros
\DeclareMathOperator{\ac}{\textnormal{c}} % constants
\DeclareMathOperator{\ad}{\textnormal{d}} % constants
\DeclareMathOperator{\ee}{\textnormal{e}} % constants
\DeclareMathOperator{\ap}{\textnormal{p}} % Probability
\DeclareMathOperator{\aq}{\textnormal{q}} % Probability
\DeclareMathOperator{\ar}{\textnormal{r}} % Probability
\DeclareMathOperator{\bK}{\textbf{K}} % Covariance matrix
\DeclareMathOperator{\cA}{\mathcal{A}} % Real numbers
\DeclareMathOperator{\cB}{\mathcal{B}} % Real numbers
\DeclareMathOperator{\cP}{\mathcal{P}} %
\DeclareMathOperator{\cS}{\mathcal{S}} %
\DeclareMathOperator{\SO}{\textnormal{SO}} % constants
\DeclareMathOperator{\sphere}{\mathbb{S}} % sphere
\DeclareMathOperator{\xb}{\mathbf{x}} % bold vector
\DeclareMathOperator{\Xb}{\mathbf{X}} % bold vector
\DeclareMathOperator{\Vb}{\mathbf{V}} % bold vector
\DeclareMathOperator{\Wb}{\mathbf{W}} % bold vector


\DeclareMathOperator{\one}{\mathbf{1}} % indicator function
\DeclareMathOperator{\zero}{\mathbf{0}} % indicator function
